Hi4D: 4D Instance Segmentation of Close Human Interaction

We propose Hi4D, a method and dataset for the automatic analysis of physically close human-human interaction under prolonged contact. Robustly disentangling several in-contact subjects is a challenging task due to occlusions and complex shapes. Hence, existing multi-view systems typically fuse 3D surfaces of close subjects into a single, connected mesh. To address this issue we leverage i) individually fitted neural implicit avatars; ii) an alternating optimization scheme that refines pose and surface through periods of close proximity; and iii) thus segment the fused raw scans into individual instances. From these instances we compile Hi4D dataset of 4D textured scans of 20 subject pairs, 100 sequences, and a total of more than 11K frames. Hi4D contains rich interaction-centric annotations in 2D and 3D alongside accurately registered parametric body models. We define varied human pose and shape estimation tasks on this dataset and provide results from state-of-the-art methods on these benchmarks.

==> Tables/comparision.tex <==

\begin{table}[h]
  \centering
  \begin{tabular}{lcccc}
    \toprule
     \textbf{Method} & \textbf{IoU}  $\uparrow$   &\textbf{C-}$\mathbf{L_2}$ $\downarrow$& \textbf{P2S} $\downarrow$ & \textbf{NC}  $\uparrow$   \\
    \midrule
    SMPL+D  & $0.983$          & $0.24$            & $0.30$          & $0.927$  \\  
     \midrule
       Ours  & $\mathbf{0.989}$ & $\mathbf{0.22}$   & $\mathbf{0.23}$ & $\mathbf{0.945}$ \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Quantitative Comparison.} Our method consistently outperforms the SMPL+D baseline in all metrics.}
  \label{tab: comparision_exp}
\end{table}



